Using dynamic circles and squares to visualize spatio-temporal variation

Visualizations such as bar charts, scatter plots, and objects on geographical maps often convey critical information, including exact and relative numeric values, using shapes. The choice of shape and method of encoding information is often arbitrarily, or based on convention. However, past studies have shown that the human eye can be fooled by visual representations. The Ebbinghaus illusion demonstrates that the perceived relative sizes of shapes depends on their configuration, which in turn can affect judgements, especially in visualizations like proportional symbol maps. In this study we evaluate the effects of varying the type of shapes and metrics for encoding data in visual representations on a spatio-temporal map interface. We find that some combinations of shape and metric are more conducive to accurate human judgements than others, and provide recommendations for applying these findings in future visualization designs.

==> formatting/deleteme <==

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

%Entries

@Article{Abril07,
  author        = "Patricia S. Abril and Robert Plant",
  title         = "The patent holder's dilemma: Buy, sell, or troll?",
  journal       = "Communications of the ACM",
  volume        = "50",
  number        = "1",
  month         = jan,
  year          = "2007",
  pages         = "36--44",
  doi           = "10.1145/1188913.1188915",
  url           = "http://doi.acm.org/10.1145/1219092.1219093",
  note          = "",
}

@Article{Cohen07,
  author        = "Sarah Cohen and Werner Nutt and Yehoshua Sagic",
  title         = "Deciding equivalances among conjunctive aggregate queries",
  journal       = JACM,
  articleno     = 5,
  numpages      = 50,
  volume        = 54,
  number        = 2,
  month         = apr,
  year          = 2007,
  doi           = "10.1145/1219092.1219093",
  url           = "http://doi.acm.org/10.1145/1219092.1219093",
  acmid         = 1219093,
}


@periodical{JCohen96,
  key =          "Cohen",
  editor =       "Jacques Cohen",
  title =        "Special issue: Digital Libraries",
  journal =      CACM,
  volume =       "39",
  number =       "11",
  month =        nov,
  year =         "1996",
}


@Book{Kosiur01,
  author =       "David Kosiur",
  title =        "Understanding Policy-Based Networking",
  publisher =    "Wiley",
  year =         "2001",
  address =      "New York, NY",
  edition =      "2nd.",
  editor =       "",
  volume =       "",
  number =       "",
  series =       "",
  month =        "",
  note =         "",
}


@Book{Harel79,
  author =       "David Harel",
  year =         "1979",
  title =        "First-Order Dynamic Logic",
  series =       "Lecture Notes in Computer Science",
  volume =       "68",
  address =      "New York, NY",
  publisher =    "Springer-Verlag",
  doi =          "10.1007/3-540-09237-4",
  url =          "http://dx.doi.org/10.1007/3-540-09237-4",
  editor =       "",
  number =       "",
  month =        "",
  note =         "",
}


@Inbook{Editor00,
  author =       "",
  editor =       "Ian Editor",
  title =        "The title of book one",
  subtitle =     "The book subtitle",
  series =       "The name of the series one",
  year =         "2007",
  volume =       "9",
  address =      "Chicago",
  edition =      "1st.",
  publisher =    "University of Chicago Press",
  doi =          "10.1007/3-540-09237-4",
  url =          "http://dx.doi.org/10.1007/3-540-09456-9",
  chapter =      "",
  pages =        "",
  number =       "",
  type =         "",
  month =        "",
  note =         "",
}

%
@InBook{Editor00a,
  author =       "",
  editor =       "Ian Editor",
  title =        "The title of book two",
  subtitle =     "The book subtitle",
  series =       "The name of the series two",
  year =         "2008",
  address =      "Chicago",
  edition =      "2nd.",
  publisher =    "University of Chicago Press",
  doi =          "10.1007/3-540-09237-4",
  url =          "http://dx.doi.org/10.1007/3-540-09456-9",
  volume =       "",
  chapter =      "100",
  pages =        "",
  number =       "",
  type =         "",
  month =        "",
  note =         "",
}


% incollection (has an editor, title, and possibly a booktitle)
@Incollection{Spector90,
  author =       "Asad Z. Spector",
  title =        "Achieving application requirements",
  booktitle =    "Distributed Systems",
  publisher =    "ACM Press",
  address =      "New York, NY",
  year =         "1990",
  edition =      "2nd.",
  chapter =      "",
  editor =       "Sape Mullender",
  pages =        "19--33",
  doi =          "10.1145/90417.90738",
  url =          "http://doi.acm.org/10.1145/90417.90738",
  volume =       "",
  number =       "",
  series =       "",
  type =         "",
  month =        "",
  note =         "",
}


% incollection (has an editor, title, and possibly a booktitle)
@Incollection{Douglass98,
  author =       "Bruce P. Douglass and David Harel and Mark B. Trakhtenbrot",
  title =        "Statecarts in use: structured analysis and object-orientation",
  series =       "Lecture Notes in Computer Science",
  booktitle =    "Lectures on Embedded Systems",
  publisher =    "Springer-Verlag",
  address =      "London",
  volume =       "1494",
  year =         "1998",
  chapter =      "",
  editor =       "Grzegorz Rozenberg and Frits W. Vaandrager",
  pages =        "368--394",
  doi =          "10.1007/3-540-65193-4_29",
  url =          "http://dx.doi.org/10.1007/3-540-65193-4_29",
  edition =      "",
  number =       "",
  type =         "",
  month =        "",
  note =         "",
}


@Book{Knuth97,
  author =       "Donald E. Knuth",
  title =        "The Art of Computer Programming, Vol. 1: Fundamental Algorithms (3rd. ed.)",
  publisher =    "Addison Wesley Longman Publishing Co., Inc.",
  year =         "1997",
  address =      "",
  edition =      "",
  editor =       "",
  volume =       "",
  number =       "",
  series =       "",
  month =        "",
  note =         "",
}


@Book{Knuth98,
  author =       "Donald E. Knuth",
  year =         "1998",
  title =        "The Art of Computer Programming",
  series =       "Fundamental Algorithms",
  volume =       "1",
  edition =      "3rd",
  address =      "",
  publisher =    "Addison Wesley Longman Publishing Co., Inc.",
  doi =          "",
  url =          "",
  editor =       "",
  number =       "",
  month =        "",
  note =         "(book)",
}

%Inbook{Knuth97,
%  author =       "Donald E. Knuth",
%  title =        "The Art of Computer Programming",
%  booktitle =    "the booktitle",
%  edition =      "3",
%  volume =       "1",
%  year =         "1997",
%  publisher =    "Addison Wesley Longman Publishing Co., Inc.",
%  editor =       "",
%  number =       "",
%  series =       "Fundamental Algorithms",
%  type =         "",
%  chapter =      "",
%  pages =        "",
%  address =      "",
%  month =        "",
%  note =         "(inbook)",
%}

%INBOOK{DK:73-inbook-full,
%   author = "Donald E. Knuth",
%   title = "Fundamental Algorithms (inbook w series)",
%   volume = 1,
%   series = "The Art of Computer Programming",
%   publisher = "Addison-Wesley",
%   address = "Reading, Massachusetts",
%   edition = "Second",
%   month = "10~" # jan,
%   year = "1973",
%   type = "Section",
%   chapter = "1.2",
%   pages = "10--119",
%   note = "Full INBOOK entry (w series)",
%}

%INcollection{DK:74-incoll,
%   author = "Donald E. Knuth",
%   title = "Fundamental Algorithms (incoll)",
%   volume = 1,
%   booktitle = "The Art of Computer Programming",
%   publisher = "Addison-Wesley",
%   address = "Reading, Massachusetts",
%   month = "10~" # jan,
%   year = "1974",
%   pages = "10--119",
%   editor = "Bernard Rous",
%   note = "This is a full incoll entry with an editor",
%}

%INcollection{DK:75-incollws,
%   author = "Donald E. Knuth",
%   title = "Fundamental Algorithms (incoll w series)",
%   volume = 1,
%   booktitle = "The Art of Computer Programming",
%   series = "The Art of Computer Programming",
%   publisher = "Addison-Wesley",
%   address = "Reading, Massachusetts",
%   month = "10~" # jan,
%   year = "1975",
%   pages = "10--119",
%   editor = "Bernard Rous",
%   note = "This is a full incoll entry with an editor and series",
%}


@incollection{GM05,
Author= "Dan Geiger and Christopher Meek",
Title= "Structured Variational Inference Procedures and their Realizations (as incol)",
Year= 2005,
Booktitle="Proceedings of Tenth International Workshop on Artificial Intelligence and Statistics, {\rm The Barbados}",
Publisher="The Society for Artificial Intelligence and Statistics",
Month= jan,
Editors= "Z. Ghahramani and R. Cowell"
}

@Inproceedings{Smith10,
  author =       "Stan W. Smith",
  title =        "An experiment in bibliographic mark-up: Parsing metadata for XML export",
  booktitle =    "Proceedings of the 3rd. annual workshop on Librarians and Computers",
  series =       "LAC '10",
  editor =       "Reginald N. Smythe and Alexander Noble",
  volume =       "3",
  year =         "2010",
  publisher =    "Paparazzi Press",
  address =      "Milan Italy",
  pages =        "422--431",
  doi =          "99.9999/woot07-S422",
  url =          "http://dx.doi.org/99.0000/woot07-S422",
  number =       "",
  month =        "",
  organization = "",
  note =         "",
}

@Inproceedings{VanGundy07,
  author =       "Matthew Van Gundy and Davide Balzarotti and Giovanni Vigna",
  year =         2007,
  title =        "Catch me, if you can: Evading network signatures with web-based polymorphic worms",
  booktitle =    "Proceedings of the first USENIX workshop on Offensive Technologies",
  series =       "WOOT '07",
  publisher =    "USENIX Association",
  address =      "Berkley, CA",
  articleno =    {Paper 7},
  numpages =     9,
}

@Inproceedings{VanGundy08,
  author =       "Matthew Van Gundy and Davide Balzarotti and Giovanni Vigna",
  year =         2008,
  title =        "Catch me, if you can: Evading network signatures with web-based polymorphic worms",
  booktitle =    "Proceedings of the first USENIX workshop on Offensive Technologies",
  series =       "WOOT '08",
  publisher =    "USENIX Association",
  address =      "Berkley, CA",
  articleno =    7,
  numpages =     2,
  pages =        "99-100",
}

@Inproceedings{VanGundy09,
  author =       "Matthew Van Gundy and Davide Balzarotti and Giovanni Vigna",
  year =         2009,
  title =        "Catch me, if you can: Evading network signatures with web-based polymorphic worms",
  booktitle =    "Proceedings of the first USENIX workshop on Offensive Technologies",
  series =       "WOOT '09",
  publisher =    "USENIX Association",
  address =      "Berkley, CA",
  pages =        "90--100",
}

@Inproceedings{Andler79,
  author =       "Sten Andler",
  title =        "Predicate Path expressions",
  booktitle =    "Proceedings of the 6th. ACM SIGACT-SIGPLAN symposium on Principles of Programming Languages",
  series =       "POPL '79",
  year =         "1979",
  publisher =    "ACM Press",
  address =      "New York, NY",
  pages =        "226--236",
  doi =          "10.1145/567752.567774",
  url =          "http://doi.acm.org/10.1145/567752.567774",
  editor =       "",
  volume =       "",
  number =       "",
  month =        "",
  organization = "",
  note =         "",
}

@Techreport{Harel78,
  author =       "David Harel",
  year =         "1978",
  title =        "LOGICS of Programs: AXIOMATICS and DESCRIPTIVE POWER",
  institution =  "Massachusetts Institute of Technology",
  type =         "MIT Research Lab Technical Report",
  number =       "TR-200",
  address =      "Cambridge, MA",
  month =        "",
  note =         "",
}

@MASTERSTHESIS{anisi03,
author = {David A. Anisi},
title = {Optimal Motion Control of a Ground Vehicle},
school = {Royal Institute of Technology (KTH), Stockholm, Sweden},
intitution = {FOI-R-0961-SE, Swedish Defence Research Agency (FOI)},
year = {2003},
}


@Phdthesis{Clarkson85,
  author =       "Kenneth L. Clarkson",
  year =         "1985",
  title =        "Algorithms for Closest-Point Problems (Computational Geometry)",
  school =       "Stanford University",
  address =      "Palo Alto, CA",
  note =         "UMI Order Number: AAT 8506171",
  type =         "",
  month =        "",
}


@online{Thornburg01,
  author =       "Harry Thornburg",
  year =         "2001",
  title =        "Introduction to Bayesian Statistics",
  url =          "http://ccrma.stanford.edu/~jos/bayes/bayes.html",
  month =        mar,
  lastaccessed = "March 2, 2005",
}


@online{Ablamowicz07,
  author =       "Rafal Ablamowicz and Bertfried Fauser",
  year =         "2007",
  title =        "CLIFFORD: a Maple 11 Package for Clifford Algebra Computations, version 11",
  url =          "http://math.tntech.edu/rafal/cliff11/index.html",
  lastaccessed = "February 28, 2008",
}


@misc{Poker06,
  author =       "Poker-Edge.Com",
  year =         "2006",
  month =        mar,
  title =        "Stats and Analysis",
  lastaccessed = "June 7, 2006",
  url =          "http://www.poker-edge.com/stats.php",
}

@misc{Obama08,
  author        = "Barack Obama",
  year          = "2008",
  title         = "A more perfect union",
  howpublished  = "Video",
  day           = "5",
  url           = "http://video.google.com/videoplay?docid=6528042696351994555",
  month         = mar,
  lastaccessed  = "March 21, 2008",
  note          =  "",
}

@misc{JoeScientist001,
  author =       "Joseph Scientist",
  year =         "2009",
  title =        "The fountain of youth",
  note =         "Patent No. 12345, Filed July 1st., 2008, Issued Aug. 9th., 2009",
  url =          "",
  howpublished = "",
  month =        aug,
  lastaccessed = "",
}


@Inproceedings{Novak03,
  author =       "Dave Novak",
  title =        "Solder man",
  booktitle =    "ACM SIGGRAPH 2003 Video Review on Animation theater Program: Part I - Vol. 145 (July 27--27, 2003)",
  year =         "2003",
  publisher =    "ACM Press",
  address =      "New York, NY",
  pages =        "4",
  month =        "March 21, 2008",
  doi =          "99.9999/woot07-S422",
  url =          "http://video.google.com/videoplay?docid=6528042696351994555",
  note =         "",
  howpublished = "Video",
  editor =       "",
  volume =       "",
  number =       "",
  series =       "",
  organization = "",
  distinctURL = 1
}


@article{Lee05,
  author =       "Newton Lee",
  year =         "2005",
  title =        "Interview with Bill Kinder: January 13, 2005",
  journal =      "Comput. Entertain.",
  eid =          "4",
  volume =       "3",
  number =       "1",
  month =        "Jan.-March",
  doi =          "10.1145/1057270.1057278",
  url =          "http://doi.acm.org/10.1145/1057270.1057278",
  howpublished = "Video",
  note =         "",
}

@article{rous08,
  author =       "Bernard Rous",
  year =         "2008",
  title =        "The Enabling of Digital Libraries",
  journal =      "Digital Libraries",
  volume =       "12",
  number =       "3",
  month =        jul,
  articleno =    "Article~5",
  doi =          "",
  url =          "",
  howpublished = "",
  note =         "To appear",
}

@article{384253,
 author = {Werneck,, Renato and Setubal,, Jo\~{a}o and da Conceic\~{a}o,, Arlindo},
 title = {(old) Finding minimum congestion spanning trees},
 journal = {J. Exp. Algorithmics},
 volume = {5},
 year = {2000},
 issn = {1084-6654},
 pages = {11},
 doi = {http://doi.acm.org/10.1145/351827.384253},
 publisher = {ACM},
 address = {New York, NY, USA},
 }


@article{Werneck:2000:FMC:351827.384253,
 author = {Werneck, Renato and Setubal, Jo\~{a}o and da Conceic\~{a}o, Arlindo},
 title = {(new) Finding minimum congestion spanning trees},
 journal = {J. Exp. Algorithmics},
 volume = 5,
 month = dec,
 year = 2000,
 issn = {1084-6654},
 articleno = 11,
 url = {http://portal.acm.org/citation.cfm?id=351827.384253},
 doi = {10.1145/351827.384253},
 acmid = 384253,
 publisher = {ACM},
 address = {New York, NY, USA},
}

@article{1555162,
 author = {Conti, Mauro and Di Pietro, Roberto and Mancini, Luigi V. and Mei, Alessandro},
 title = {(old) Distributed data source verification in wireless sensor networks},
 journal = {Inf. Fusion},
 volume = {10},
 number = {4},
 year = {2009},
 issn = {1566-2535},
 pages = {342--353},
 doi = {http://dx.doi.org/10.1016/j.inffus.2009.01.002},
 publisher = {Elsevier Science Publishers B. V.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@article{Conti:2009:DDS:1555009.1555162,
 author = {Conti, Mauro and Di Pietro, Roberto and Mancini, Luigi V. and Mei, Alessandro},
 title = {(new) Distributed data source verification in wireless sensor networks},
 journal = {Inf. Fusion},
 volume = {10},
 number = {4},
 month = oct,
 year = {2009},
 issn = {1566-2535},
 pages = {342--353},
 numpages = {12},
 url = {http://portal.acm.org/citation.cfm?id=1555009.1555162},
 doi = {10.1016/j.inffus.2009.01.002},
 acmid = {1555162},
 publisher = {Elsevier Science Publishers B. V.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Clone detection, Distributed protocol, Securing data fusion, Wireless sensor networks},
}

@inproceedings{Li:2008:PUC:1358628.1358946,
 author = {Li, Cheng-Lun and Buyuktur, Ayse G. and Hutchful, David K. and Sant, Natasha B. and Nainwal, Satyendra K.},
 title = {Portalis: using competitive online interactions to support aid initiatives for the homeless},
 booktitle = {CHI '08 extended abstracts on Human factors in computing systems},
 year = {2008},
 isbn = {978-1-60558-012-X},
 location = {Florence, Italy},
 pages = {3873--3878},
 numpages = {6},
 url = {http://portal.acm.org/citation.cfm?id=1358628.1358946},
 doi = {10.1145/1358628.1358946},
 acmid = {1358946},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {cscw, distributed knowledge acquisition, incentive design, online games, recommender systems, reputation systems, user studies, virtual community},
}

@book{Hollis:1999:VBD:519964,
 author = {Hollis, Billy S.},
 title = {Visual Basic 6: Design, Specification, and Objects with Other},
 year = {1999},
 isbn = {0130850845},
 edition = {1st},
 publisher = {Prentice Hall PTR},
 address = {Upper Saddle River, NJ, USA},
 }


@book{Goossens:1999:LWC:553897,
 author = {Goossens, Michel and Rahtz, S. P. and Moore, Ross and Sutor, Robert S.},
 title = {The  Latex Web Companion: Integrating TEX, HTML, and XML},
 year = {1999},
 isbn = {0201433117},
 edition = {1st},
 publisher = {Addison-Wesley Longman Publishing Co., Inc.},
 address = {Boston, MA, USA},
 }

% need to test genres for errant isbn output

% techreport
@techreport{897367,
 author = {Buss, Jonathan F. and Rosenberg, Arnold L. and Knott, Judson D.},
 title = {Vertex Types in Book-Embeddings},
 year = {1987},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Aumass_cs%3Ancstrl.umassa_cs%2F%2FUM-CS-1987-018},
 publisher = {University of Massachusetts},
 address = {Amherst, MA, USA},
 }

@techreport{Buss:1987:VTB:897367,
 author = {Buss, Jonathan F. and Rosenberg, Arnold L. and Knott, Judson D.},
 title = {Vertex Types in Book-Embeddings},
 year = {1987},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Aumass_cs%3Ancstrl.umassa_cs%2F%2FUM-CS-1987-018},
 publisher = {University of Massachusetts},
 address = {Amherst, MA, USA},
 }

% whole proceedings

@proceedings{Czerwinski:2008:1358628,
 author = {},
 note = {General Chair-Czerwinski, Mary and General Chair-Lund, Arnie and Program Chair-Tan, Desney},
 title = {CHI '08: CHI '08 extended abstracts on Human factors in computing systems},
 year = {2008},
 isbn = {978-1-60558-012-X},
 location = {Florence, Italy},
 order_no = {608085},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

% phdthesis

@phdthesis{Clarkson:1985:ACP:911891,
 author = {Clarkson, Kenneth Lee},
 advisor = {Yao, Andrew C.},
 title = {Algorithms for Closest-Point Problems (Computational Geometry)},
 year = {1985},
 note = {AAT 8506171},
 school = {Stanford University},
 address = {Stanford, CA, USA},
 }
% school is being picked up -- but not publisher (which is OK)
% Also -- the title is NOT being output in italics !!! Arrrrgh! - I fixed it. :-)


%%% compare with 'old'
%%% atsign-Phdthesis{Clarkson85,
%%%  author =       "Kenneth L. Clarkson",
%%%  year =         "1985",
%%%  title =        "Algorithms for Closest-Point Problems (Computational Geometry)",
%%%  school =       "Stanford University",
%%%  address =      "Palo Alto, CA",
%%%  note =         "UMI Order Number: AAT 8506171",
%%%  type =         "",
%%%  month =        "",
%%%}

% A bibliography
@Article{1984:1040142,
 key = {{$\!\!$}},
 journal = {SIGCOMM Comput. Commun. Rev.},
 year = {1984},
 issn = {0146-4833},
 volume = {13-14},
 number = {5-1},
 issue_date = {January/April 1984},
 publisher = {ACM},
 address = {New York, NY, USA},
 }


% grinder
@inproceedings{2004:ITE:1009386.1010128,
 key = {IEEE},
 title = {IEEE TCSC Executive Committee},
 booktitle = {Proceedings of the IEEE International Conference on Web Services},
 series = {ICWS '04},
 year = {2004},
 isbn = {0-7695-2167-3},
 pages = {21--22},
 url = {http://dx.doi.org/10.1109/ICWS.2004.64},
 doi = {http://dx.doi.org/10.1109/ICWS.2004.64},
 acmid = {1010128},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
}

% div book
@book{Mullender:1993:DS:302430,
 editor = {Mullender, Sape},
 title = {Distributed systems (2nd Ed.)},
 year = {1993},
 isbn = {0-201-62427-3},
 publisher = {ACM Press/Addison-Wesley Publishing Co.},
 address = {New York, NY, USA},
 }

% master thesis (as techreport and thesis)

@techreport{Petrie:1986:NAD:899644,
 author = {Petrie, Charles J.},
 title = {New Algorithms for Dependency-Directed Backtracking (Master's thesis)},
 year = {1986},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Autexas_cs%3AUTEXAS_CS%2F%2FAI86-33},
 publisher = {University of Texas at Austin},
 address = {Austin, TX, USA},
 }

@MASTERSTHESIS{Petrie:1986:NAD:12345,
 author = {Petrie, Charles J.},
 title = {New Algorithms for Dependency-Directed Backtracking (Master's thesis)},
 year = {1986},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Autexas_cs%3AUTEXAS_CS%2F%2FAI86-33},
 school = {University of Texas at Austin},
 address = {Austin, TX, USA},
 }




@BOOK{book-minimal,
   author = "Donald E. Knuth",
   title = "Seminumerical Algorithms",
   publisher = "Addison-Wesley",
   year = "1981",
}

% incollection (has an editor, title, and possibly a booktitle)
@INcollection{KA:2001,
 author = {Kong, Wei-Chang},
 Title = {The implementation of electronic commerce in SMEs in Singapore (as Incoll)},
 booktitle = {E-commerce and cultural values},
 year = {2001},
 isbn = {1-59140-056-2},
 pages = {51--74},
 numpages = {24},
 url = {http://portal.acm.org/citation.cfm?id=887006.887010},
 acmid = {887010},
 publisher = {IGI Publishing},
 address = {Hershey, PA, USA},
}


% with bibfield 'type' before chapter (note no editor)
@INBOOK{KAGM:2001,
 author = {Kong, Wei-Chang},
 type = {Name of Chapter:},
 chapter = {The implementation of electronic commerce in SMEs in Singapore (Inbook-w-chap-w-type)},
 title = {E-commerce and cultural values},
 year = {2001},
 isbn = {1-59140-056-2},
 pages = {51--74},
 numpages = {24},
 url = {http://portal.acm.org/citation.cfm?id=887006.887010},
 acmid = {887010},
 publisher = {IGI Publishing},
 address = {Hershey, PA, USA},
}

%%% Notes! This is because the atsign-INBOOK citation type specifies EITHER
%%% editor or author, but not both. In my experiments with the harvard/dcu
%%% bibtex style (and presumably this applies to other styles too), bibtex
%%% ignores the editor information if author information exists in an
%%% atsign-INBOOK entry. atsign-INCOLLECTION is far more commonly used in my references,
%%% and in the absence of an editor I believe most bibtex styles will just
%%% ommit the editor from the reference - the chapter information will not
%%% end up in the in-text citation as you suggest it should be but at least
%%% there is a place to put the editor if necessary.



% was 'Inbook' -- changed to incollection - (editor is different to author) - need to tell Asad to codify as such.
@incollection{Kong:2002:IEC:887006.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {Chapter 9},
  booktitle =   {E-commerce and cultural values (Incoll-w-text (chap 9) 'title')},
  year =        {2002},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  type =        "",
  month =       "",
  note =        "",
}

% incol when the chapter is 'text' - due to presence of editor (different to author)
@incollection{Kong:2003:IEC:887006.887011,
 author = {Kong, Wei-Chang},
 title = {The implementation of electronic commerce in SMEs in Singapore (Incoll)},
 booktitle = {E-commerce and cultural values},
 editor = {Thanasankit, Theerasak},
 year = {2003},
 isbn = {1-59140-056-2},
 pages = {51--74},
 numpages = {24},
 url = {http://portal.acm.org/citation.cfm?id=887006.887010},
 acmid = {887010},
 publisher = {IGI Publishing},
 address = {Hershey, PA, USA},
}

% ------ test
%incollection{Kong:2003:IEC:887006.887010,
% author = {Kong, Wei-Chang},
% chapter = {The implementation of electronic commerce in SMEs in Singapore (Incoll-text-in-chap)},
% booktitle = {booktitle E-commerce and cultural values},
% title =   {The title},
% editor = {Thanasankit, Theerasak},
% year = {2003},
% isbn = {1-59140-056-2},
% pages = {51--74},
% numpages = {24},
% url = {http://portal.acm.org/citation.cfm?id=887006.887010},
% acmid = {887010},
% publisher = {IGI Publishing},
% address = {Hershey, PA, USA},
%}


% ---------





% Need inbook with num in chapter

% and inbook with number in chapter
@InBook{Kong:2004:IEC:123456.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {E-commerce and cultural values - (InBook-num-in-chap)},
  chapter =     {9},
  year =        {2004},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  type =        "",
  month =       "",
  note =        "",
}


% and inbook with text in chapter
@Inbook{Kong:2005:IEC:887006.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {E-commerce and cultural values (Inbook-text-in-chap)},
  chapter =     {The implementation of electronic commerce in SMEs in Singapore},
  year =        {2005},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  type =        {Chapter:},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  month =       "",
  note =        "",
}


% and inbook with a num and type field
@Inbook{Kong:2006:IEC:887006.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {E-commerce and cultural values (Inbook-num chap)},
  chapter =     {22},
  year =        {2006},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  type =        {Chapter (in type field)},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  month =       "",
  note =        "",
}


% and incol coz we have a BLANK chapter - due to presence of editor
%atIncollection{Kong:2006:IEC:887006.887011,
%  author =     {Kong, Wei-Chang},
%  editor =     {Theerasak Thanasankit},
%  title =      "The title"
%  booktitle =  {E-commerce and cultural values (Incol-coz-blank-chap)},
%  year =       {2006},
%  address =    {Hershey, PA, USA},
%  publisher =  {IGI Publishing},
%  url =        {http://portal.acm.org/citation.cfm?id=887006.887010},
%  type =       {Type!},
%  chapter =    {},
%  pages =      {51--74},
%  numpages =   {24},
%  acmid =      {887010},
%  isbn =       {1-59140-056-2},
%  number =     "",
%  month =      "",
%  note =       "",
%}

@article{SaeediMEJ10,
            author = {Mehdi Saeedi and Morteza Saheb Zamani and Mehdi Sedighi},
            title = {A library-based synthesis methodology for reversible logic},
            journal = {Microelectron. J.},
            volume = {41},
            number = {4},
            month = apr,
            year = {2010},
            pages = {185--194},
}

@ARTICLE{SaeediJETC10,
            author = {Mehdi Saeedi and Morteza Saheb Zamani and Mehdi Sedighi and Zahra Sasanian},
            title = {Synthesis of Reversible Circuit Using Cycle-Based Approach},
            journal = {J. Emerg. Technol. Comput. Syst.},
            volume = {6},
            number = {4},
            month = dec,
            year = {2010}
            }

% Asad's new version
@article{Kirschmer:2010:AEI:1958016.1958018,
 author = {Kirschmer, Markus and Voight, John},
 title = {Algorithmic Enumeration of Ideal Classes for Quaternion Orders},
 journal = {SIAM J. Comput.},
 issue_date = {January 2010},
 volume = {39},
 number = {5},
 month = jan,
 year = {2010},
 issn = {0097-5397},
 pages = {1714--1747},
 numpages = {34},
 url = {http://dx.doi.org/10.1137/080734467},
 doi = {https://doi.org/10.1137/080734467},
 acmid = {1958018},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
 keywords = {ideal classes, maximal orders, number theory, quaternion algebras},
}


% incol due to presence of booktitle
@incollection{Hoare:1972:CIN:1243380.1243382,
 author = {Hoare, C. A. R.},
 title = {Chapter II: Notes on data structuring},
 booktitle = {Structured programming (incoll)},
 editor = {Dahl, O. J. and Dijkstra, E. W. and Hoare, C. A. R.},
 year = {1972},
 isbn = {0-12-200550-3},
 pages = {83--174},
 numpages = {92},
 url = {http://portal.acm.org/citation.cfm?id=1243380.1243382},
 acmid = {1243382},
 publisher = {Academic Press Ltd.},
 address = {London, UK, UK},
}

% incol due to presence of booktitle
@incollection{Lee:1978:TQA:800025.1198348,
 author = {Lee, Jan},
 title = {Transcript of question and answer session},
 booktitle = {History of programming languages I (incoll)},
 editor = {Wexelblat, Richard L.},
 year = {1981},
 isbn = {0-12-745040-8},
 pages = {68--71},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/800025.1198348},
 doi = {http://doi.acm.org/10.1145/800025.1198348},
 acmid = {1198348},
 publisher = {ACM},
 address = {New York, NY, USA},
}

% incol due to booktitle
@incollection{Dijkstra:1979:GSC:1241515.1241518,
 author = {Dijkstra, E.},
 title = {Go to statement considered harmful},
 booktitle = {Classics in software engineering (incoll)},
 year = {1979},
 isbn = {0-917072-14-6},
 pages = {27--33},
 numpages = {7},
 url = {http://portal.acm.org/citation.cfm?id=1241515.1241518},
 acmid = {1241518},
 publisher = {Yourdon Press},
 address = {Upper Saddle River, NJ, USA},
}

% incol due to booktitle
@incollection{Wenzel:1992:TVA:146022.146089,
 author = {Wenzel, Elizabeth M.},
 title = {Three-dimensional virtual acoustic displays},
 booktitle = {Multimedia interface design (incoll)},
 year = {1992},
 isbn = {0-201-54981-6},
 pages = {257--288},
 numpages = {32},
 url = {http://portal.acm.org/citation.cfm?id=146022.146089},
 doi = {10.1145/146022.146089},
 acmid = {146089},
 publisher = {ACM},
 address = {New York, NY, USA},
}

% incol due to booktitle
@incollection{Mumford:1987:MES:54905.54911,
 author = {Mumford, E.},
 title = {Managerial expert systems and organizational change: some critical research issues},
 booktitle = {Critical issues in information systems research (incoll)},
 year = {1987},
 isbn = {0-471-91281-6},
 pages = {135--155},
 numpages = {21},
 url = {http://portal.acm.org/citation.cfm?id=54905.54911},
 acmid = {54911},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
}

@book{McCracken:1990:SSC:575315,
 author = {McCracken, Daniel D. and Golden, Donald G.},
 title = {Simplified Structured COBOL with Microsoft/MicroFocus COBOL},
 year = {1990},
 isbn = {0471514071},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
}

% Let's include Boris / BBeeton entries  (multi-volume works)

@book {MR781537,
    AUTHOR = {H{\"o}rmander, Lars},
     TITLE = {The analysis of linear partial differential operators. {III}},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {275},
      NOTE = {Pseudodifferential operators},
PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin, Germany},
      YEAR = {1985},
     PAGES = {viii+525},
      ISBN = {3-540-13828-5},
   MRCLASS = {35-02 (35Sxx 47G05 58G15)},
  MRNUMBER = {781536 (87d:35002a)},
MRREVIEWER = {Min You Qi},
}

@book {MR781536,
    AUTHOR = {H{\"o}rmander, Lars},
     TITLE = {The analysis of linear partial differential operators. {IV}},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {275},
      NOTE = {Fourier integral operators},
PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin, Germany},
      YEAR = {1985},
     PAGES = {vii+352},
      ISBN = {3-540-13829-3},
   MRCLASS = {35-02 (35Sxx 47G05 58G15)},
  MRNUMBER = {781537 (87d:35002b)},
MRREVIEWER = {Min You Qi},
}

%%%%%%%%%%%%%%%%%%%%%% Start of Aptara sample bib entries

% acmsmall-sam.bib
@InProceedings{Adya-01,
  author        = {A. Adya and P. Bahl and J. Padhye and A.Wolman and L. Zhou},
  title         = {A multi-radio unification protocol for {IEEE} 802.11 wireless networks},
  booktitle     = {Proceedings of the IEEE 1st International Conference on Broadnets Networks (BroadNets'04)},
  publisher     = "IEEE",
  address       = "Los Alamitos, CA",
  year          = {2004},
  pages         = "210--217"
}

@article{Akyildiz-01,
  author        = {I. F. Akyildiz and W. Su and Y. Sankarasubramaniam and E. Cayirci},
  title         = {Wireless Sensor Networks: A Survey},
  journal       = {Comm. ACM},
  volume        = 38,
  number        = "4",
  year          = {2002},
  pages         = "393--422"
}

@article{Akyildiz-02,
  author        = {I. F. Akyildiz and T. Melodia and K. R. Chowdhury},
  title         = {A Survey on Wireless Multimedia Sensor Networks},
  journal       = {Computer Netw.},
  volume        = 51,
  number        = "4",
  year          = {2007},
  pages         = "921--960"
}

@InProceedings{Bahl-02,
  author        = {P. Bahl and R. Chancre and J. Dungeon},
  title         = {{SSCH}: Slotted Seeded Channel Hopping for Capacity Improvement in {IEEE} 802.11 Ad-Hoc Wireless Networks},
  booktitle     = {Proceeding of the 10th International Conference on Mobile Computing and Networking (MobiCom'04)},
  publisher     = "ACM",
  address       = "New York, NY",
  year          = {2004},
  pages         = "112--117"
}

@misc{CROSSBOW,
  key       = {CROSSBOW},
  title     = {{XBOW} Sensor Motes Specifications},
  note      = {http://www.xbow.com},
  year      = 2008
}

@article{Culler-01,
  author        = {D. Culler and D. Estrin and M. Srivastava},
  title         = {Overview of Sensor Networks},
  journal       = {IEEE Comput.},
  volume        = 37,
  number        = "8 (Special Issue on Sensor Networks)",
  publisher     = "IEEE",
  address       = "Los Alamitos, CA",
  year          = {2004},
  pages         = "41--49"
}

@misc{Harvard-01,
    key         = {Harvard CodeBlue},
    title       = {{CodeBlue}: Sensor Networks for Medical Care},
    note        = {http://www.eecs.harvard.edu/mdw/ proj/codeblue/},
    year        = 2008
}

@InProceedings{Natarajan-01,
    author      = {A. Natarajan and M. Motani and B. de Silva and K. Yap and K. C. Chua},
    title       = {Investigating Network Architectures for Body Sensor Networks},
    booktitle   = {Network Architectures},
    editor      = {G. Whitcomb and P. Neece},
    publisher   = "Keleuven Press",
    address     = "Dayton, OH",
    year        = {2007},
    pages       = "322--328",
    eprint      = "960935712",
    primaryclass = "cs",
}

@techreport{Tzamaloukas-01,
  author        = {A. Tzamaloukas and J. J. Garcia-Luna-Aceves},
  title         = {Channel-Hopping Multiple Access},
  number =        {I-CA2301},
  institution =   {Department of Computer Science, University of California},
  address =       {Berkeley, CA},
  year          = {2000}
}

@BOOK{Zhou-06,
  author        = {G. Zhou and J. Lu and C.-Y. Wan and M. D. Yarvis and J. A. Stankovic},
  title         = {Body Sensor Networks},
  publisher     = "MIT Press",
  address       = "Cambridge, MA",
  year          = {2008}
}

@mastersthesis{ko94,
author = "Jacob Kornerup",
title = "Mapping Powerlists onto Hypercubes",
school = "The University of Texas at Austin",
note = "(In preparation)",
year = "1994"}
%month = "dec",}

@PhdThesis{gerndt:89,
  author =       "Michael Gerndt",
  title =        "Automatic Parallelization for Distributed-Memory
                  Multiprocessing Systems",
  school =       "University of Bonn",
  year =         1989,
  address =      "Bonn, Germany",
  month =        dec
}

@article{6:1:1,
author = "J. E. {Archer, Jr.} and R. Conway and F. B. Schneider",
title = "User recovery and reversal in interactive systems",
journal = "ACM Trans. Program. Lang. Syst.",
volume =  "6",
number = "1",
month = jan,
year = 1984,
pages = "1--19"}

@article{7:1:137,
author = "D. D. Dunlop and V. R. Basili",
title = "Generalizing specifications for uniformly implemented loops",
journal = "ACM Trans. Program. Lang. Syst.",
volume =  "7",
number = "1",
month = jan,
year = 1985,
pages = "137--158"}

@article{7:2:183,
author = "J. Heering and P. Klint",
title = "Towards monolingual programming environments",
journal = "ACM Trans. Program. Lang. Syst.",
volume =  "7",
number = "2",
month = apr,
year = 1985,
pages = "183--213"}

@book{knuth:texbook,
author = "Donald E. Knuth",
title = "The {\TeX{}book}",
publisher = "Addison-Wesley",
address = "Reading, MA.",
year = 1984}

@article{6:3:380,
author = "E. Korach and D.  Rotem and N. Santoro",
title = "Distributed algorithms for finding centers and medians in networks",
journal = "ACM Trans. Program. Lang. Syst.",
volume =  "6",
number = "3",
month = jul,
year = 1984,
pages = "380--401"}

@book{Lamport:LaTeX,
author = "Leslie Lamport",
title = "\it {\LaTeX}: A Document Preparation System",
publisher = "Addison-Wesley",
address = "Reading, MA.",
year = 1986}

@article{7:3:359,
author = "F. Nielson",
title = "Program transformations in a denotational setting",
journal = "ACM Trans. Program. Lang. Syst.",
volume =  "7",
number = "3",
month = jul,
year = 1985,
pages = "359--379"}

%testing
@BOOK{test,
   author = "Donald E. Knuth",
   title = "Seminumerical Algorithms",
   volume = 2,
   series = "The Art of Computer Programming",
   publisher = "Addison-Wesley",
   address = "Reading, MA",
   edition = "2nd",
   month = "10~" # jan,
   year = "1981",
}

@inproceedings{reid:scribe,
author = "Brian K. Reid",
title = "A high-level approach to computer document formatting",
booktitle = "Proceedings of the 7th Annual Symposium on Principles of
  Programming Languages",
month = jan,
year = 1980,
publisher = "ACM",
address = "New York",
pages = "24--31"}

@article{Zhou:2010:MMS:1721695.1721705,
 author = {Zhou, Gang and Wu, Yafeng and Yan, Ting and He, Tian and Huang, Chengdu and Stankovic, John A. and Abdelzaher, Tarek F.},
 title = {A multifrequency MAC specially designed for wireless sensor network applications},
 journal = {ACM Trans. Embed. Comput. Syst.},
 issue_date = {March 2010},
 volume = 9,
 number = 4,
 month = {April},
 year = 2010,
 issn = {1539-9087},
 pages = {39:1--39:41},
 articleno = 39,
 numpages = 41,
 url = {http://doi.acm.org/10.1145/1721695.1721705},
 doi = {10.1145/1721695.1721705},
 acmid = 1721705,
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Wireless sensor networks, media access control, multi-channel, radio interference, time synchronization},
}


@online{TUGInstmem,
  key =          {TUG},
  year  =        2017,
  title =        "Institutional members of the {\TeX} Users Group",
  url =          "http://wwtug.org/instmem.html",
  lastaccessed = "May 27, 2017",
}

@online{CTANacmart,
  author =    {Boris Veytsman},
  title =  {acmart---{C}lass for typesetting publications of {ACM}},
  year = 2017,
  url =    {http://www.ctan.org/pkg/acmart},
  lastaccessed = {May 27, 2017}
  }

@ARTICLE{bowman:reasoning,
    author = {Bowman, Mic and Debray, Saumya K. and Peterson, Larry L.},
    title = {Reasoning About Naming Systems},
    journal = {ACM Trans. Program. Lang. Syst.},
    volume = {15},
    number = {5},
    pages = {795-825},
    month = {November},
    year = {1993},
    doi = {10.1145/161468.161471},
}

@ARTICLE{braams:babel,
    author = {Braams, Johannes},
    title = {Babel, a Multilingual Style-Option System for Use with LaTeX's Standard Document Styles},
    journal = {TUGboat},
    volume = {12},
    number = {2},
    pages = {291-301},
    month = {June},
    year = {1991},
}

@INPROCEEDINGS{clark:pct,
  AUTHOR = "Malcolm Clark",
  TITLE = "Post Congress Tristesse",
  BOOKTITLE = "TeX90 Conference Proceedings",
  PAGES = "84-89",
  ORGANIZATION = "TeX Users Group",
  MONTH = "March",
  YEAR = {1991}
}

@ARTICLE{herlihy:methodology,
    author = {Herlihy, Maurice},
    title = {A Methodology for Implementing Highly Concurrent Data Objects},
    journal = {ACM Trans. Program. Lang. Syst.},
    volume = {15},
    number = {5},
    pages = {745-770},
    month = {November},
    year = {1993},
    doi = {10.1145/161468.161469},
}

@BOOK{salas:calculus,
  AUTHOR = "S.L. Salas and Einar Hille",
  TITLE = "Calculus: One and Several Variable",
  PUBLISHER = "John Wiley and Sons",
  ADDRESS = "New York",
  YEAR = "1978"
}

@MANUAL{Fear05,
  title =        {Publication quality tables in {\LaTeX}},
  author =       {Simon Fear},
  month =        {April},
  year =         2005,
  note =         {\url{http://www.ctan.org/pkg/booktabs}}
}

@Manual{Amsthm15,
  title =        {Using the amsthm Package},
  organization = {American Mathematical Society},
  month =        {April},
  year =         2015,
  note =         {\url{http://www.ctan.org/pkg/amsthm}}
}

@ArtifactSoftware{R,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2019},
    url = {https://www.R-project.org/},
}

@ArtifactDataset{UMassCitations,
 author    =  {Sam Anzaroot and Andrew McCallum},
 title     =  {{UMass} Citation Field Extraction Dataset},
 year      = 2013,
 url       =
    {http://www.iesl.cs.umass.edu/data/data-umasscitationfield},
 lastaccessed = {May 27, 2019}
}

@Eprint{Bornmann2019,
       author = {Bornmann, Lutz and Wray, K. Brad and Haunschild,
                  Robin},
        title = {Citation concept analysis {(CCA)}---A new form of
                  citation analysis revealing the usefulness of
                  concepts for other researchers illustrated by two
                  exemplary case studies including classic books by
                  {Thomas S.~Kuhn} and {Karl R.~Popper}},
     keywords = {Computer Science - Digital Libraries},
         year = 2019,
        month = "May",
          eid = {arXiv:1905.12410},
archivePrefix = {arXiv},
       eprint = {1905.12410},
 primaryClass = {cs.DL},
}

@Eprint{AnzarootPBM14,
  author    = {Sam Anzaroot and
               Alexandre Passos and
               David Belanger and
               Andrew McCallum},
  title     = {Learning Soft Linear Constraints with Application to
                  Citation Field Extraction},
  year      = {2014},
  archivePrefix = {arXiv},
  eprint    = {1403.1349},
}

@inproceedings{Hagerup1993,
title        = {Maintaining Discrete Probability Distributions Optimally},
author       = {Hagerup, Torben and Mehlhorn, Kurt and Munro, J. Ian},
booktitle    = {Proceedings of the 20th International Colloquium on Automata, Languages and Programming},
series       = {Lecture Notes in Computer Science},
volume       = {700},
pages        = {253--264},
year         = {1993},
publisher    = {Springer-Verlag},
address      = {Berlin},
}

